Real-world Video Adaptation with Reinforcement Learning

Client-side video players employ adaptive bitrate (ABR) algorithms to optimize user quality of experience (QoE). We evaluate recently proposed RL-based ABR methods in Facebook's web-based video streaming platform. Real-world ABR contains several challenges that requires customized designs beyond off-the-shelf RL algorithms -- we implement a scalable neural network architecture that supports videos with arbitrary bitrate encodings; we design a training method to cope with the variance resulting from the stochasticity in network conditions; and we leverage constrained Bayesian optimization for reward shaping in order to optimize the conflicting QoE objectives. In a week-long worldwide deployment with more than 30 million video streaming sessions, our RL approach outperforms the existing human-engineered ABR algorithms.

==> related.tex <==
\section{Related Work}
\label{s:related}
%
The earliest ABR approaches can be primarily grouped into rate-based and buffer-based
algorithms. Rate-based algorithms \cite{festive,cs2p} estimate the available network throughput
using past observation of the network statistics, and then request video chunks at the highest
bitrate that the network is predicted to support.
%
For example, Festive~\cite{festive} predicts bandwidth to be the harmonic mean
of the experienced throughput for the past 5 chunk downloads. 
%
These methods are constrained by the accuracy of bandwidth prediction on top of
HTTP~\cite{cfa,panda}.
%
Several work aims to improve throughput estimates using smoothing heuristics and data aggregation
techniques~\cite{cs2p}, but making these algorithms robust still remains a challenge
in practice~\cite{hotmobile15}.
%
On the other hand, buffer-based approaches~\cite{teyuansig,bola} decide the bitrates for future chunks
based on the video playback buffer occupancy. The idea of these algorithms is to maintain
the buffer at a certain pre-configured level to make cushion for the risk of stalls.
%
As a recent buffer-based approach, BOLA~\cite{bola}, optimizes for a specified QoE
metric using a Lyapunov optimization formulation. 


These two approaches have their own strength: the rate-based approaches work well best
when link rates are stable and can provide initial ABR suggestions at startup time,
while the buffer-based approaches are more robust in steady state and in the presence of
time-varying networks~\cite{teyuansig}.
%
More recent work consider merging both observations in a unified ABR framework.
%
For example, robustMPC~\cite{mpc} employs model predictive control algorithms that uses current buffer 
condition and a conservative estimation of future throughput to select bitrates that are expected to maximize QoE over a horizon of several future chunks. 
%
However, this approach relies heavily on accurate throughput estimates which are not always available.
%
When throughput predictions are incorrect, the ABR performance can degrade significantly~\cite{pensieve}.

There has been several studies on applying RL to adaptive video streaming~\cite{pensieve, oboe} with
fixed set of network traces in controlled settings.
%
These methods train and tailor the ABR algorithm to optimize for the specific network characteristics in
deployment.
%
Our work is largely built on top of Pensieve~\cite{pensieve}, which first uses modern RL approach to
train high-quality ABR algorithms that outperform all prior approaches.
%
Beyond off-the-shelf RL methods, we add several specialized components when designing \name to solve
the unique challenges in deployment (\S\ref{s:design}).
%
Similar to the self improving methodology in RL, Oboe~\cite{oboe} recently proposes a learning approach
to automatically tune the parameters in existing ABR algorithms (e.g., the buffer threshold for switching
to higher bitrates in buffer-based algorithms).
%
In \name, we use Bayesian optimization to tune the reward weights to shape the optimization objective
in order to outperform the existing production ABR algorithm.

%Recently there have been a surge of work applying RL to other networked computer systems.
%
%For example, auto, decima, tf device placement, 
%


